Adaptive Latent Entity Expansion for Document Retrieval

Despite considerable progress in neural relevance ranking techniques, search engines still struggle to process complex queries effectively - both in terms of precision and recall. Sparse and dense Pseudo-Relevance Feedback (PRF) approaches have the potential to overcome limitations in recall, but are only effective with high precision in the top ranks. In this work, we tackle the problem of search over complex queries using three complementary techniques. First, we demonstrate that applying a strong neural re-ranker before sparse or dense PRF can improve the retrieval effectiveness by 5-8%. This improvement in PRF effectiveness can be attributed directly to improving the precision of the feedback set. Second, we propose an enhanced expansion model, Latent Entity Expansion (LEE), which applies fine-grained word and entity-based relevance modelling incorporating localized features. Specifically, we find that by including both words and entities for expansion achieve a further 2-8% improvement in NDCG. Our analysis also demonstrated that LEE is largely robust to its parameters across datasets and performs well on entity-centric queries. And third, we include an 'adaptive' component in the retrieval process, which iteratively refines the re-ranking pool during scoring using the expansion model and avoids re-ranking additional documents. We find that this combination of techniques achieves the best NDCG, MAP and R@1000 results on the TREC Robust 2004 and CODEC document datasets, demonstrating a significant advancement in expansion effectiveness.

==> tables/corpus_entities.tex <==
\begin{table}[b]
\caption{Corpus statistics - including average number of non-stop words and WAT entity links per document.}
\label{tab:corpus-entities}
\begin{tabular}{l|c|c|c|}
\cline{2-4}
                               & \multicolumn{1}{l|}{Documents} & \multicolumn{1}{l|}{Av. Words} & \multicolumn{1}{l|}{Av. Entities} \\ \hline
\multicolumn{1}{|l|}{Robust04} & 528,155                   & 332.5                          & 116.0                         \\ \hline
\multicolumn{1}{|l|}{CODEC}    & 729,824                   & 466.1                          & 159.6      \\ \hline
% \multicolumn{1}{|l|}{Core18}   & 595,031                   & 361.1                          & 117.9                         \\ \hline
\end{tabular}
\end{table}

==> tables/entity_queries.tex <==
\begin{table}[h!]
\label{tab:entity-queries}
\caption{How entities queries impact retrieval}
\begin{tabular}{l|c|ccc|}
\cline{2-5}
                                      & \multicolumn{1}{c|}{Entity Rank} & \multicolumn{3}{c|}{Document Rank} \\ \cline{2-5} 
                                      & NDCG@20                          & NDCG      & MAP      & R@1000      \\ \hline
\multicolumn{1}{|l|}{RM3-ent}         &                                  &           &          &             \\
\multicolumn{1}{|l|}{Graph-IQ-Degree} &                                  &           &          &             \\
\multicolumn{1}{|l|}{Graph-IQ-Eigen}  &                                  &           &          &             \\
\multicolumn{1}{|l|}{Graph-IQ-Walk}   &                                  &           &          &             \\
\multicolumn{1}{|l|}{CODEC-ent-qrels} &                                  &           &          &             \\ \hline
\end{tabular}
\end{table}

==> tables/graph_rerank.tex <==
\begin{table}[h!]
\caption{Graph-IQ re-ranking effectiveness. All methods use BM25+RM3 input system for consistency, except EQFE that uses a fused initial run \cite{dalton2014entity}. (++) indicates systems that are fine-tuned on target datasets. (*) indicates 5\% paired-t-test significance against BM25+RM3 \textgreater{}\textgreater T5-3b system.}
\label{tab:graph-rerank}
\begin{tabular}{l|cc|cc|}
\cline{2-5}
                                                              & \multicolumn{2}{c|}{Title}      & \multicolumn{2}{c|}{Description} \\ \cline{2-5} 
                                                              & NDCG@20        & NDCG           & NDCG@20         & NDCG           \\ \hline
\multicolumn{1}{|l|}{BM25+RM3}                                & 0.435          & 0.571          & 0.425           & 0.551          \\
\multicolumn{1}{|l|}{EQFE}                                    & 0.431          & 0.601          & -               & -              \\
\multicolumn{1}{|l|}{Entity-Aspects}                          &                &                &                 &                \\
\multicolumn{1}{|l|}{BERT-FirstP}                             & 0.455          & 0.569          & 0.470           & 0.564          \\
\multicolumn{1}{|l|}{BERT-MaxP}                               & 0.485          & 0.599          & 0.492           & 0.591          \\
\multicolumn{1}{|l|}{T5-base}                                 & 0.485          & 0.601          & 0.525           & 0.611          \\
\multicolumn{1}{|l|}{T5-3b}                                   & 0.536          & 0.634          & 0.605           & 0.652          \\ \hline
\multicolumn{1}{|l|}{GAR-BM25}                                & 0.535          & 0.641          & 0.610           & 0.670          \\
\multicolumn{1}{|l|}{GAR-ColBERT}                             & 0.535          & 0.645          & 0.606           & 0.669          \\
\multicolumn{1}{|l|}{Graph-IQ (No KG)}                        & 0.536          & 0.658          & 0.612           & 0.693          \\
\multicolumn{1}{|l|}{Graph-IQ}                                & 0.563          & \textbf{0.669} & 0.624           & \textbf{0.696} \\ \hline
\multicolumn{1}{|l|}{CEDR**}                                  & 0.547          & 0.632          & 0.598           & 0.645          \\
\multicolumn{1}{|l|}{PARADE**}                                & 0.566          & 0.642          & 0.613           & 0.650          \\
\multicolumn{1}{|l|}{MORES**}                                 & \textbf{0.569} & -              & \textbf{0.641}  & -              \\
\multicolumn{1}{|l|}{Graph-IQ\textgreater{}\textgreater{}P**} &                &                &                 &                \\
\multicolumn{1}{|l|}{Graph-IQ+P**}                            &                &                &                 &                \\ \hline
\end{tabular}
\end{table}

==> tables/graphs_methods.tex <==
\begin{table*}[h!]
\caption{Graph-IQ initial retrieval effectiveness. All Graph-IQ and GAR methods using BM25+RM3 input run for consistency. (*) indicates 5\% paired-t-test significance against BM25+RM3 \textgreater{}\textgreater T5-3b system.}
\label{tab:graph-methods}
\begin{tabular}{l|ccc|ccc|ccc|}
\cline{2-10}
                                                                       & \multicolumn{3}{c|}{Robust04 - Title}            & \multicolumn{3}{c|}{Robust04 - Description}      & \multicolumn{3}{c|}{CODEC}                       \\ \cline{2-10} 
                                                                       & NDCG           & MAP            & R@1000         & NDCG           & MAP            & R@1000         & NDCG           & MAP            & R@1000         \\ \hline
\multicolumn{1}{|l|}{ColBERT-TCT \textgreater{}\textgreater T5-3b}     & 0.561          & 0.327          & 0.637          & 0.564          & 0.346          & 0.595          & 0.602          & 0.348          & 0.740          \\
\multicolumn{1}{|l|}{ColBERT-TCT+PRF \textgreater{}\textgreater T5-3b} & 0.582          & 0.344          & 0.677          & 0.570          & 0.356          & 0.615          & 0.603          & 0.350          & 0.744          \\
\multicolumn{1}{|l|}{ENT-Dense \textgreater{}\textgreater T5-3b}       & 0.498          & 0.290          & 0.537          & 0.514          & 0.309          & 0.526          & 0.585          & 0.333          & 0.706          \\
\multicolumn{1}{|l|}{ENT-Sparse \textgreater{}\textgreater T5-3b}      & 0.598          & 0.357          & 0.714          & 0.640          & 0.397          & 0.722          & 0.637          & 0.372          & 0.809          \\
\multicolumn{1}{|l|}{ENT-Sparse+PRF \textgreater{}\textgreater T5-3b}  & 0.615          & 0.366          & 0.745          & 0.658          & 0.407          & 0.759          & 0.647          & 0.373          & 0.833          \\
\multicolumn{1}{|l|}{BM25 \textgreater{}\textgreater T5-3b}            & 0.594          & 0.351          & 0.705          & 0.603          & 0.375          & 0.664          & 0.632          & 0.372          & 0.783          \\
\multicolumn{1}{|l|}{BM25+RM3 \textgreater{}\textgreater T5-3b}        & 0.634          & 0.377          & 0.777          & 0.652          & 0.406          & 0.750          & 0.644          & 0.377          & 0.816          \\ \hline
\multicolumn{1}{|l|}{GAR-BM25}                                         & 0.641          & 0.380          & 0.787          & 0.670          & 0.414          & 0.779          & 0.646          & 0.375          & 0.817          \\
\multicolumn{1}{|l|}{GAR-ColBERT}                                      & 0.645          & 0.384          & 0.796          & 0.669          & 0.414          & 0.774          & 0.638          & 0.371          & 0.816          \\ \hline
\multicolumn{1}{|l|}{Graph-IQ-Degree}                                  & 0.638          & 0.380          & 0.783          & 0.662          & 0.410          & 0.767          & 0.653          & 0.374          & 0.853          \\
\multicolumn{1}{|l|}{Graph-IQ-Walk}                                    & 0.656          & 0.387          & 0.819          & 0.693          & 0.428          & \textbf{0.817} & 0.656          & 0.375          & 0.860          \\
\multicolumn{1}{|l|}{Graph-IQ-EdgeW}                                   & 0.658          & 0.389          & \textbf{0.821} & 0.693          & 0.429          & \textbf{0.817} & 0.657          & 0.376          & \textbf{0.861} \\ \hline
\multicolumn{1}{|l|}{Graph-IQ}                                         & \textbf{0.669} & \textbf{0.405} & \textbf{0.821} & \textbf{0.696} & \textbf{0.437} & \textbf{0.817} & \textbf{0.668} & \textbf{0.385} & \textbf{0.861} \\ \hline
\end{tabular}
\end{table*}

==> tables/latency.tex <==
\begin{table}[h!]
\caption{Latency.}
\label{tab:latency}
\begin{tabular}{l|ll|l|}
\cline{2-4}
                           & Graph-IQ & T5-3b & Total Time \\ \hline
\multicolumn{1}{|l|}{100}  &          &       &            \\ \cline{1-1}
\multicolumn{1}{|l|}{500}  &          &       &            \\ \cline{1-1}
\multicolumn{1}{|l|}{1000} &          &       &            \\ \hline
\end{tabular}
\end{table}

==> tables/ndcg_all_systems.tex <==
\begin{table*}[h!]
\caption{NDCG@20 comparing initial retrieval systems re-ranked with T5-3b versus re-ranked with Graph-IQ. (*) indicates 5\% paired-t-test significance against T5-3b and Graph-IQ.}
\label{tab:ndcg-all-systems}
\begin{tabular}{l|ccc|ccc|ccc|}
\cline{2-10}
                                      & \multicolumn{3}{c|}{Robust04 - Title} & \multicolumn{3}{c|}{Robust04 - Description} & \multicolumn{3}{c|}{CODEC}      \\ \cline{2-10} 
                                      & T5-3b   & Graph-IQ         & \%       & T5-3b     & Graph-IQ           & \%         & T5-3b & Graph-IQ       & \%     \\ \hline
\multicolumn{1}{|l|}{ColBERT-TCT}     & 0.524   & 0.561            & +7.1\%   & 0.589     & 0.619              & +5.1\%     & 0.482 & 0.505          & +4.8\% \\
\multicolumn{1}{|l|}{ColBERT-TCT+PRF} & 0.530   & 0.562            & +6.0\%   & 0.575     & 0.616              & +7.1\%     & 0.478 & 0.502          & +5.0\% \\
\multicolumn{1}{|l|}{ENT-Dense}       & 0.496   & 0.556            & +12.1\%  & 0.559     & 0.609              & +8.9\%     & 0.466 & 0.499          & +7.1\% \\
\multicolumn{1}{|l|}{ENT-Sparse}      & 0.532   & 0.565            & +6.2\%   & 0.612     & 0.631              & +3.1\%     & 0.490 & 0.514          & +4.9\% \\
\multicolumn{1}{|l|}{ENT-Sparse+PRF}  & 0.530   & 0.563            & +6.2\%   & 0.607     & \textbf{0.632}     & +4.1\%     & 0.490 & 0.510          & +4.1\% \\
\multicolumn{1}{|l|}{BM25}            & 0.532   & 0.563            & +5.8\%   & 0.602     & 0.630              & +4.7\%     & 0.498 & 0.513          & +3.0\% \\
\multicolumn{1}{|l|}{BM25+RM3}        & 0.536   & 0.563            & +5.0\%   & 0.605     & 0.624              & +3.1\%     & 0.497 & 0.509          & +2.4\% \\ \hline
\multicolumn{1}{|l|}{RR-Fusion}       & 0.535   & \textbf{0.566}   & +5.8\%   & 0.608     & 0.627              & +3.1\%     & 0.491 & \textbf{0.515} & +4.9\% \\ \hline
\end{tabular}
\end{table*}

==> tables/queries_entities.tex <==
\begin{table}[b]
\caption{Query statistics - including average number of non-stop words and ELQ entity links per query}
\label{tab:queries-entities}
\begin{tabular}{l|c|c|c|}
\cline{2-4}
                                             & \multicolumn{1}{l|}{Topics} & \multicolumn{1}{l|}{Av. Words} & \multicolumn{1}{l|}{Av. Entities} \\ \hline
\multicolumn{1}{|l|}{Robust04 - Title}       & 249                         & 2.7                              & 1.5                             \\ \hline
\multicolumn{1}{|l|}{Robust04 - Description} & 249                         & 15.4                             & 5.3     \\ \hline
\multicolumn{1}{|l|}{CODEC}                  & 42                          & 10.5                             & 4.1    \\ \hline
% \multicolumn{1}{|l|}{Core18 - title}         & 50                          & 3.1                              & 1.5                             \\ \hline
% \multicolumn{1}{|l|}{Core18 - description}   & 50                          & 15.5                             & 4.7                             \\ \hline
\end{tabular}
\end{table}

==> tables/recall_all_systems.tex <==

\begin{table*}[h!]
\caption{Recall@1000 comparing solely initial retrieval systems (Original) with each system when combined with Graph-IQ. (*) indicates 5\% paired-t-test significance against Original and Graph-IQ.}
\label{tab:recall-all-systems}
\begin{tabular}{l|ccc|ccc|ccc|}
\cline{2-10}
                                      & \multicolumn{3}{c|}{Robust04 - Title} & \multicolumn{3}{c|}{Robust04 - Description} & \multicolumn{3}{c|}{CODEC}       \\ \cline{2-10} 
                                      & T5-3b   & Graph-IQ         & \%       & T5-3b     & Graph-IQ           & \%         & T5-3b & Graph-IQ       & \%      \\ \hline
\multicolumn{1}{|l|}{ColBERT-TCT}     & 0.637   & 0.794            & +24.6\%  & 0.595     & 0.789              & +32.6\%    & 0.740 & 0.855          & +15.5\% \\
\multicolumn{1}{|l|}{ColBERT-TCT+PRF} & 0.681   & 0.799            & +17.3\%  & 0.656     & 0.778              & +18.6\%    & 0.775 & 0.866          & +11.7\% \\
\multicolumn{1}{|l|}{ENT-Dense}       & 0.537   & 0.750            & +39.7\%  & 0.526     & 0.751              & +42.8\%    & 0.706 & 0.830          & +17.6\% \\
\multicolumn{1}{|l|}{ENT-Sparse}      & 0.714   & 0.804            & +12.6\%  & 0.722     & 0.818              & +13.3\%    & 0.809 & 0.874          & +8.0\%  \\
\multicolumn{1}{|l|}{ENT-Sparse+PRF}  & 0.745   & 0.806            & +8.2\%   & 0.759     & 0.820              & +8.0\%     & 0.833 & 0.868          & +4.2\%  \\
\multicolumn{1}{|l|}{BM25}            & 0.705   & 0.819            & +16.2\%  & 0.664     & 0.808              & +21.7\%    & 0.783 & 0.870          & +11.1\% \\
\multicolumn{1}{|l|}{BM25+RM3}        & 0.777   & 0.821            & +5.7\%   & 0.750     & 0.817              & +8.9\%     & 0.816 & 0.861          & +5.5\%  \\ \hline
\multicolumn{1}{|l|}{RR-Fusion}       & 0.814   & \textbf{0.842}   & +3.4\%   & 0.786     & \textbf{0.834}     & +6.1\%     & 0.879 & \textbf{0.892} & +1.5\%  \\ \hline
\end{tabular}
\end{table*}
